On bounded Wang tilings

Wang tiles enable efficient pattern compression while avoiding the periodicity in tile distribution via programmable matching rules. However, most research in Wang tilings has considered tiling the infinite plane. Motivated by emerging applications in materials engineering, we consider the bounded version of the tiling problem and offer four integer programming formulations to construct valid or nearly-valid Wang tilings: a decision, maximum-rectangular tiling, maximum cover, and maximum adjacency constraint satisfaction formulations. To facilitate a finer control over the resulting tilings, we extend these programs with tile-based, color-based, packing, and variable-sized periodic constraints. Furthermore, we introduce an efficient heuristic algorithm for the maximum-cover variant based on the shortest path search in directed acyclic graphs and derive simple modifications to provide a $1/2$ approximation guarantee for arbitrary tile sets, and a $2/3$ guarantee for tile sets with cyclic transducers. Finally, we benchmark the performance of the integer programming formulations and of the heuristic algorithms showing that the heuristics provides very competitive outputs in a fraction of time. As a by-product, we reveal errors in two well-known aperiodic tile sets: the Knuth tile set contains a tile unusable in two-way infinite tilings, and the Lagae corner tile set is not aperiodic.

==> tiles/removed <==
\hide{
\begin{proposition}\label{prop:0.5}
	Assuming an arbitrary tile set $\mathcal{T}$, Algorithm \ref{alg:simple} terminates with at least $0.5 \lvert \mathcal{A}\rvert$ placed tiles.
	\begin{proof}
		To show this, we start by tiling the first row. In the worst-case, the tile set $\mathcal{T}$ contains tiles with mutually incompatible edge colors, e.g., 
		%
		\begin{equation*}
		\mathcal{T} = 
		\left\{ 
		\WangTile{$0$}{$0$}{$1$}{$1$}
		\right\}.
		\end{equation*}
		%
		In this case, the algorithm generates the tile-void-tile-\dots (or reversed) pattern, rendering the number of placed tiles equal to $\lceil0.5\lvert \mathcal{W} \rvert\rceil$, where $\lceil \bullet \rceil$ denotes rounding of $\bullet$ to the nearest greater-or-equal integer.
		
		Second, we prove that the number of tiles in any two consecutive rows is $\lvert\mathcal{W}\rvert$ at least. Hence, let us now consider tiling of the $i$-th row when the $(i-1)$-th row is already tiled. To this goal, there are two options:
		%
		\begin{enumerate}
			\item \textit{The $(i-1)$-th row contains alternating void and tile sequences, and the length of all the void sequences is at most $p_{\max,\mathrm{h}}$}, where $p_{\max,\mathrm{h}}$ denotes the longest path in the transducer $G_{\mathrm{t},\mathrm{h}}$. Then, we can always populate the $i$-th row positions that are below the voids of the $(i-1)$-th row. Thus, we have at least $\lvert \mathcal{W} \rvert$ placed tiles.
			%
			\begin{figure*}[!htbp]
				\centering
				\begin{minipage}{0.3\linewidth}
					\centering
					$\mathcal{T} = \left\{ \WangTile{0}{0}{1}{1}, \WangTile{0}{1}{1}{2} \right\}$
				\end{minipage}%
				\begin{minipage}{0.7\linewidth}
					\centering
					\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\vspace{-0.5mm}\\
					{\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile}
				\end{minipage}
			\end{figure*}
			
			Notice that this case also applies to the setting when the $(i-1)$-th row is full void. In such case, the row $(i-2)\ge1$ must be fully covered, i.e., $p_{\max, \mathrm{h}}=\lvert \mathcal{H} \rvert$, as we could place a tile at the $(i-1)$-th row otherwise. Hence, also the $i$-th row must be fully covered.
			%
			\item \textit{The $(i-1)$-th row contains alternating void and tile strings, and the length of the void sequence is greater than $p_{\max,\mathrm{h}}$}. To prove this setting, we first show that the void sequence length is bounded by $p_{\max,\mathrm{h}}+2$ from above. Considering a~triplet of tile positions $\{(i-1,j-1),(i-1,j),(i-1,j+1)\}$ with a void placed at $(i-1,j)$, we can always put a~tile at $(i,j)$ regardless of the content of $(i-1,j-1)$ and $(i-1,j+1)$. Indeed, placing a~tile at any of $\{(i-1,j), (i+1,j)\}$ may prevent appearance of a tile at $(i,j)$ due to the edge-matching rules. However, at least a single position in $\{(i,j-1),(i,j),(i,j+1)\}$ must be occupied by a tile to maintain the maximum-row-cover property.
			
			From point $1$ it follows that the length of the void sequences may be in the range $\{1,\dots,p_{\max,\mathrm{h}}\}$. The longest sequence is formed by inserting the widest valid row tiling (of length $p_{\max,\mathrm{h}}$) into the $(i-2)$-th row. If the south color codes of these tiles do possess any outgoing arcs in the dual transducer graph, there indeed does not exist any tile that can be connected; we have at least a $p_{\max,\mathrm{h}}$-wide void sequence. However, because the valid tiling sequence at the $(i-2)$-th row is the widest, its west and east neighbors must be voids. Based on the former reasoning, there must be a tile placed near these voids. In the worst case, a tile may be placed at the southwest of the west void and southeast of the east one. Altogether, this produces a sequence of at most $p_{\max,\mathrm{h}}+2$ voids in the $(i-1)$-th row. 
			
			Let us now consider a tiling of the $(i-1)$-th row by
			\begin{figure*}[!htbp]
			$p_1$ tiles - $v_1$ voids - $p_2$ tiles - $v_2$ voids - \dots - $p_n$ tiles - $v_n$ voids
			\end{figure*}
			
			Based on 1., we can clearly place tiles to the south of all void sequences of the length at most $p_{\max,\mathrm{h}}$. For void sequences of the length $p_{\max,\mathrm{h}}+1$, only $p_{\max,\mathrm{h}}$ tiles can be used. Similarly, the void sequences of the length $p_{\max,\mathrm{h}}+2$ allow us to insert at least $p_{\max,\mathrm{h}}+1$ tiles, i.e., by using the sequence $p_{\max,\mathrm{h}}$ tiles - $1$ void - $1$ tile. Hence, for any of these longer void sequences at the $(i-1)$-th we may lose a single tile at the $i$-th row.
			%\begin{figure*}[!htbp]
			%	\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\vspace{-0.5mm}\\
			%	{\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\WangTile{0}{0}{1}{1}\hspace{-0.25mm}\WangTile{0}{1}{1}{3}\hspace{-0.25mm}\EmptyTile\hspace{-0.25mm}\EmptyTile}
			%\end{figure*}			
		\end{enumerate}
	
		\todo{
		\begin{itemize}
			\item $(i-2)$-th row: 
		\end{itemize}
		}
		
		Now assume that a tiling of the $i$-th row is generated. Then, the tiling of the $(i+1)$-th row will form  either a tile-void-tile-void-\dots, or void-tile-void-tile-\dots pattern, such that the patterns of the $i$-th and $i+1$-th rows are inverted. Therefore, any two consecutive rows contain at least $\lvert \mathcal{W} \rvert$ tiles. 
		
		Consequently, the pattern of the first row appears $\lceil 0.5 \lvert \mathcal{H} \rvert \rceil$ times in the tiling, in every odd row, and the other pattern appears in $\lfloor 0.5 \lvert \mathcal{H} \rvert \rfloor$ instances. Thus,
		%
		\begin{equation}
		\lvert \mathcal{B_{\mathrm{cov}}} \rvert \ge \lceil 0.5 \lvert \mathcal{H} \rvert \rceil \lceil 0.5\lvert \mathcal{W} \rvert \rceil + \lfloor 0.5 \lvert \mathcal{H} \rvert \rfloor \lfloor 0.5\lvert \mathcal{W} \rvert \rfloor \ge 0.5\lvert \mathcal{A} \rvert.
		\end{equation}
	\end{proof}
\end{proposition}

\begin{proposition}
	The approximation ratio of Algorithm~\ref{alg:simple} is $0.5$.
	\begin{proof}
		In Proposition~\ref{prop:0.5}, we have shown that $\lvert \mathcal{B_{\mathrm{cov}}} \rvert \ge 0.5 \lvert \mathcal{A} \rvert$. It rests to be shown that this bound is tight even for tile sets that allow for valid tiling of $\mathcal{A}$.
		
		Consider the tile set
		%
		\begin{equation*}
		\mathcal{T} = 
		\left\{ 
		\WangTile{$0$}{$1$}{$1$}{$1$},\;
		\WangTile{$2$}{$2$}{$2$}{$2$}
		\right\}.
		\end{equation*}
		%
		Clearly, the tile set allows for tiling the infinite plane using the second tile only, so that $\lvert\mathcal{B_{\max \mathrm{cov}}} \rvert = \lvert \mathcal{A} \rvert$. Algorithm~\ref{alg:simple} may output, however, odd rows tiled by the first tile and the other rows by voids, because none of the tiles can be placed there. If $\lvert \mathcal{H} \rvert$ is even, the tiling will contain exactly $0.5 \lvert \mathcal{A} \rvert$ tiles, i.e., $\lvert \mathcal{B_{\mathrm{cov}}} \rvert = 0.5\lvert \mathcal{A}\rvert$.
	\end{proof}
\end{proposition}}
